Accelerated, Optimal, and Parallel: Some Results on Model-Based Stochastic Optimization

We extend the Approximate-Proximal Point (aProx) family of model-based methods for solving stochastic convex optimization problems, including stochastic subgradient, proximal point, and bundle methods, to the minibatch and accelerated setting. To do so, we propose specific model-based algorithms and an acceleration scheme for which we provide non-asymptotic convergence guarantees, which are order-optimal in all problem-dependent constants and provide linear speedup in minibatch size, while maintaining the desirable robustness traits (e.g. to stepsize) of the aProx family. Additionally, we show improved convergence rates and matching lower bounds identifying new fundamental constants for "interpolation" problems, whose importance in statistical machine learning is growing; this, for example, gives a parallelization strategy for alternating projections. We corroborate our theoretical results with empirical testing to demonstrate the gains accurate modeling, acceleration, and minibatching provide.

==> proofs.tex <==
\section{Technical Results}
\label{proof:sec:non-asym}
\begin{lemma}(\emph{Fenchel Young inequality})\label{lem:fenchel-young}
For any convex function $f(\cdot)$, let $f\opt(\cdot)$ denote its Fenchel dual. Then, we have 
\begin{equation}
f(x) + f\opt(y) \geq x^Ty.
\end{equation}
\end{lemma}
Specifically, we use the following two instances of Fenchel-Young extensively: 
\begin{enumerate}
    \item For $f(x) = \frac{\ltwo{x}^2}{2\beta}$, we have $f\opt(y) =  \frac{\beta}{2}\ltwo{y}^2$ for any constant $\beta > 0$. Thus, we obtain
    \begin{equation*}
     x^Ty  \leq \frac{1}{2\beta}\ltwo{x}^2 + \frac{\beta}{2}\ltwo{y}^2.
    \end{equation*}
    \item For $f(x) = \frac{x^TMx}{2}$, we have $f\opt(y) =  \frac{y^TM^{-1}y}{2}$ for any positive definite matrix $M$. Thus, we have
    \begin{equation*}
        x^Ty \leq \frac{x^TMx}{2} + \frac{y^TM^{-1}y}{2}.
    \end{equation*}
\end{enumerate}

% \subsection{Proof of \Cref{lem:smooth_progress}}
% \label{proof:lem:smooth_progress}


% \subsection{Proof of \Cref{thm:non-asym-variance}}
% \label{proof:thm:non-asym-variance}

% \subsection{Proof of \Cref{thm:full-prox}}
% \label{proof:thm:full-prox}




% \subsection{Proof of \Cref{thm:accel-rate}}
% \label{proof:thm:accel-rate}


% \subsection{Proof of \Cref{cor:accel-result}}
% \label{proof:cor:accel-result}

% \section{Proofs of \Cref{sec:interpolation}}



% \subsection{Proof of \Cref{thm:easysharpgrowth}}
% WLOG let $f(x\opt) = 0$. We define $D_k := \dist(x_k, \domain\opt)$ and $\xi_k := \grad F(x_k; \statrv_k) - \grad f(x_k)$ and $\lambda_k := \min(2\alpha_k, f(x_k)/\left\|\nabla f(x_k)\right\|_{2}^2)$. We begin with \cref{eq:prequel3.1} and apply \Cref{lem:fenchel-young}:
% \begin{align*}
% \frac{1}{2}D_{k+1}^2 &\leq \frac{1}{2} D_k^2 + \alpha_k [f(x\opt) - f(x_{k+1})] - \frac{1}{2}\left\|x_k  - x_{k+1}\right\|_{2}^2 + \alpha_k e_k \\
% & + \alpha_k \langle \xi_k, x_k - x_{k+1}\rangle + \frac{\alpha_k L}{2} \left\|x_k - x_{k+1}\right\|_{2}^2\\
% &\leq \frac{1}{2} D_k^2 + \alpha_k [f(x\opt) - f(x_{k+1})] - \frac{1}{2}\left\|x_k  - x_{k+1}\right\|_{2}^2 + \alpha_k e_k \\
% & + \frac{\alpha_k}{\eta_k 2} \left\|\xi_k\right\|_{2}^2  +  \frac{\alpha_k (L + \eta_k)}{2} \left\|x_k - x_{k+1}\right\|_{2}^2\\
% &= \frac{1}{2} D_k^2 - \alpha_k f(x_{k+1}) -  \frac{1}{4} \left\|x_k - x_{k+1}\right\|_{2}^2+ \alpha_k e_k +\frac{\alpha_k}{2 \eta_k}\left\|\xi_{k}\right\|_{2}^2  \\
% &\hspace*{8cm} \text{(Choosing $\alpha_k = \frac{1}{2}(L + \eta_k)^{-1}$)}
% \end{align*}
% Observe that due to convexity and our assumption that $f(x\opt) = 0$, we have that $ f(x_{k+1}) \geq [f(x_{k}) + \langle \nabla f(x_k), x_{k+1} - x_k\rangle]_+$, meaning that
% \begin{align*}
% \frac{1}{2}D_{k+1}^2 &\leq \frac{1}{2} D_k^2 - \alpha_k [f(x_{k}) + \langle \nabla f(x_k), x_{k+1} - x_k\rangle]_+ -  \frac{1}{4} \left\|x_k - x_{k+1}\right\|_{2}^2+ \alpha_k e_k +\frac{\alpha_k}{2 \eta_k}\left\|\xi_{k}\right\|_{2}^2\\
% &= \frac{1}{2} D_k^2 - (\alpha_k[f(x_{k}) + \langle \nabla f(x_k), x_{k+1} - x_k\rangle]_+ +  \frac{1}{4}\left\|x_k - x_{k+1}\right\|_{2}^2)+ \alpha_k e_k +\frac{\alpha_k}{2 \eta_k}\left\|\xi_{k}\right\|_{2}^2\\
% &\leq \frac{1}{2} D_k^2 -  (\min_y\alpha_k[f(x_{k}) + \langle \nabla f(x_k), y - x_k\rangle]_+ + \frac{1}{4} \left\|x_k -y\right\|_{2}^2)+ \alpha_k e_k +\frac{\alpha_k}{2 \eta_k}\left\|\xi_{k}\right\|_{2}^2\\
% &= \frac{1}{2} D_k^2 - (\alpha_k[f(x_{k}) - \lambda_k \| \nabla f(x_k)\|_2^2] +  \frac{\lambda_k^2}{4}  \left\| \nabla f(x_k)\right\|_{2}^2)+ \alpha_k e_k +\frac{\alpha_k}{2 \eta_k}\left\|\xi_{k}\right\|_{2}^2 \\ 
% & \hspace*{8.5cm} (\text{since } y\opt = x_k - \lambda_k \nabla f(x_k))\\
% &\leq \frac{1}{2} D_k^2 -  (\frac{1}{2}\lambda_k[f(x_{k}) - \lambda_k \| \nabla f(x_k)\|_2^2] + \frac{\lambda_k^2}{4}  \left\| \nabla f(x_k)\right\|_{2}^2)+ \alpha_k e_k +\frac{\alpha_k}{2 \eta_k}\left\|\xi_{k}\right\|_{2}^2\\
% & \hspace*{10cm} (\text{since } \lambda_k \leq 2\alpha_k)\\
% &= \frac{1}{2} D_k^2 - \frac{1}{2} \lambda_k f(x_k) + \frac{\lambda_k^2}{4} \left\|\nabla f(x_k)\right\|_{2}^2+ \alpha_k e_k +\frac{\alpha_k}{2 \eta_k}\left\|\xi_{k}\right\|_{2}^2
% \end{align*}
% We proceed by cases: if $\lambda_k = f(x_k)/ \|\nabla f(x_k)\|_{2}^2$, then $- \frac{1}{2} \lambda_k f(x_k) + \frac{\lambda_k^2}{4} \|\nabla f(x_k)\|_{2}^2 = -\frac{f(x_k)^2}{4\|\nabla f(x_k)\|_{2}^2}$. If $\lambda_k = 2\alpha_k$ (by using the fact that $2\alpha_k^2 \leq \alpha_k f(x_k) / \|\nabla f(x_k)\|_{2}^2$), then $- \frac{1}{2} \lambda_k f(x_k) + \frac{\lambda_k^2}{4} \|\nabla f(x_k)\|_{2}^2 = -\alpha_k f(x_k)/ 2$. In taking an upper bound of these two cases, we get:
% \begin{align*}
% \frac{1}{2}D_{k+1}^2 &\leq \frac{1}{2} D_k^2 - \frac{1}{2} \lambda_k f(x_k) + \frac{\lambda_k^2}{4} \left\|\nabla f(x_k)\right\|_{2}^2+ \alpha_k e_k +\frac{\alpha_k}{2 \eta_k}\left\|\xi_{k}\right\|_{2}^2\\
% &\leq  \frac{1}{2} D_k^2 - \min\left(\frac{\alpha_k f(x_k)}{2} , \frac{f(x_k)^2}{4\|\nabla f(x_k)\|_{2}^2} \right)+ \alpha_k e_k +\frac{\alpha_k}{2 \eta_k}\left\|\xi_{k}\right\|_{2}^2
% \end{align*}
% Rearranging, using Assumption \ref{assm:sharp-growth-population}, and taking expectations on both sides, we get:
% \begin{align*}
%     \E[D_{k+1}^2] &\leq  \E[D_k^2] - \E\left[\min\left( \alpha_k f(x_k) , \frac{f(x_k)^2}{2\|\nabla f(x_k)\|_{2}^2} \right)\right]+ 2\alpha_k \E[e_k] +\frac{\alpha_k}{ \eta_k}\E[\|\xi_{k}\|_{2}^2]\\
%     &\leq  \left\{1 - \min\left(\lambda_0 \alpha_k, \frac{\lambda_1}{2D_k} \right)  +\frac{\alpha_k \sigma^2}{m \eta_k}\right\}\E[D_k^2] \\
%     &\leq  \left\{1 - \min\left(\lambda_0 \alpha_k, \frac{\lambda_1}{2D_1} \right)  +\frac{\alpha_k \sigma^2}{m \eta_k}\right\}\E[D_k^2]
% \end{align*}
% The second inequality comes from Assumption \ref{assm:bounded-noise-dist} and the fact that $\E[e_k] \leq 0$. Now we apply the fact that $1 - t\leq e^{-t}$ to get the expression:
% \begin{align*}
%     \E[D_{k+1}^2] &\leq \left\{1 - \min\left(\lambda_0 \alpha_k, \frac{\lambda_1}{2D_1} \right)  +\frac{\alpha_k \sigma^2}{m \eta_k}\right\}\E[D_k^2]\\
%     &\leq \exp\left\{- \min\left(\lambda_0 \alpha_k, \frac{\lambda_1}{2D_1} \right)  +\frac{\alpha_k \sigma^2}{m \eta_k}\right\}\E[D_k^2]
% \end{align*}

% Reapplying this inequality completes the proof.
\subsection{Proof of \cref{lem:gamma-growth-ub}}
\label{proof:lem:gamma-growth-ub}

Consider the event $A := \{\statval: |\Fbar'(x;\statval)|^2 \leq
2\E[|\Fbar'(x;\statval)|^2]/ p, \Fbar(x;\statval) \geq c
\dist(x,x\opt)^{1+\gamma}\}$. Notice that:
\begin{align*}
    \P(A) &\geq 1 - \P(|\Fbar'(x;\statrv_1^m)|^2 \geq 2\E[|\Fbar'(x;\statval)|^2]/ p) - \P(\Fbar(x;\statrv_1^m) \geq c \dist(x,x\opt))\\
    &\geq 1 - p/2 - (1-p) = p/2,
\end{align*}
where we use a union bound then Markov's inequality. We apply this observation to arrive at
\begin{align*}
   & \E\left[\min\left(\alpha \Fbar(x; \statrv_1^m), \frac{\Fbar(x; \statrv_1^m)^2}{ \ltwo{\Fbar'(x; \statrv_1^m)}^2}\right) \right] \\
%   \geq & \E\left[\min\left(\alpha \Fbar(x; \statrv_1^m), \frac{\Fbar(x; \statrv_1^m)^2}{ \ltwo{\Fbar'(x; \statrv_1^m)}^2}\right)\ind{A}\right] \\
   \stackrel{(i)}\geq & \frac{p}{2} \min\left(\alpha c \dist(x, \domain\opt)^{1+\gamma}, \frac{pc^2 \dist(x, \domain\opt)^{2+2\gamma}}{2\ltwo{f'(x)}^2(1 + \frac{\var(F'(x;\statrv))}{m\ltwo{f'(x)}^2})}\right)\\
    \stackrel{(ii)}\geq & \frac{p}{2} \min\left(\alpha c \dist(x, \domain\opt)^{1+\gamma}, \frac{pc^2 \dist(x, \domain\opt)^{2}}{2L^2(1 + \frac{\var(F'(x;\statrv))}{m\ltwo{f'(x)}^2})}\right)\\
    \geq & \frac{p}{2} \min\left(\alpha c , \frac{pc^2 \dist(x, \domain\opt)^{1-\gamma}}{2L^2(1 + \frac{\noisetosig}{m})}\right)\dist(x, \domain\opt)^{1+\gamma},
\end{align*}
where (i) follows from $\E[X] \geq \E[X\ind{A}]$ and (ii) follows from Condition \ref{cond:gamma-growth-sufficient2}. \proofbox

% \subsection{Proof of \Cref{lem:sharp-growth-ub}}

% Consider the event: $A := \{\statval: |\Fbar'(x;\statval)|^2 \leq 2\E[|\Fbar'(x;\statval)|^2]/ p, \Fbar(x;\statval) \geq c \dist(x,x\opt)\}$. Notice that:
% \begin{align*}
%     \P(A) &= 1-\P(A^c) \geq 1 - \P(|\Fbar'(x;\statrv_1^m)|^2 \geq 2\E[|\Fbar'(x;\statval)|^2]/ p) - \P(\Fbar(x;\statrv_1^m) \geq c \dist(x,x\opt))\\
%     &\geq 1 - p/2 - (1-p) = p/2
% \end{align*}
% where we use a union bound then Markov's inequality. Further notice that then:
% \begin{align*}
%   & \E\left[\min(\alpha \Fbar(x; \statrv_1^m), \frac{\Fbar(x; \statrv_1^m)^2}{ \ltwo{\Fbar'(x; \statrv_1^m)}^2}) \right] \\
%   \geq & \E\left[\min(\alpha \Fbar(x; \statrv_1^m), \frac{\Fbar(x; \statrv_1^m)^2}{ \ltwo{\Fbar'(x; \statrv_1^m)}^2})\ind{A}\right] \\
%   \geq & \frac{p}{2} \min\left(\alpha c \dist(x, \domain\opt), \frac{pc^2 \dist(x, \domain\opt)^2}{2(\ltwo{f'(x)}^2 + \frac{\sigma^2}{m})}\right)
% \end{align*}

% \subsection{Proof of \Cref{thm:easyquadgrowth}}
% WLOG let $f(x\opt) = 0$. We define $D_k := \dist(x_k, \domain\opt)$ and $\xi_k := \grad F(x_k; \statrv_k) - \grad f(x_k)$ and $\lambda_k := \min(2\alpha_k, f(x_k)/\left\|\nabla f(x_k)\right\|_{2}^2)$. We begin with \cref{eq:prequel3.1} and apply \Cref{lem:fenchel-young}:
% \begin{align*}
% \frac{1}{2}D_{k+1}^2 &\leq \frac{1}{2} D_k^2 + \alpha_k [f(x\opt) - f(x_{k+1})] - \frac{1}{2}\left\|x_k  - x_{k+1}\right\|_{2}^2 + \alpha_k e_k \\
% & + \alpha_k \langle \xi_k, x_k - x_{k+1}\rangle + \frac{\alpha_k L}{2} \left\|x_k - x_{k+1}\right\|_{2}^2\\
% &\leq \frac{1}{2} D_k^2 + \alpha_k [f(x\opt) - f(x_{k+1})] - \frac{1}{2}\left\|x_k  - x_{k+1}\right\|_{2}^2 + \alpha_k e_k \\
% & + \frac{\alpha_k}{\eta_k 2} \left\|\xi_k\right\|_{2}^2  +  \frac{\alpha_k (L + \eta_k)}{2} \left\|x_k - x_{k+1}\right\|_{2}^2\\
% &= \frac{1}{2} D_k^2 - \alpha_k f(x_{k+1}) -  \frac{1}{4} \left\|x_k - x_{k+1}\right\|_{2}^2+ \alpha_k e_k +\frac{\alpha_k}{2 \eta_k}\left\|\xi_{k}\right\|_{2}^2  \\
% &\hspace*{8cm} \text{(Choosing $\alpha_k = \frac{1}{2}(L + \eta_k)^{-1}$)}
% \end{align*}
% Observe that due to convexity and our assumption that $f(x\opt) = 0$, we have that $ f(x_{k+1}) \geq [f(x_{k}) + \langle \nabla f(x_k), x_{k+1} - x_k\rangle]_+$, meaning that
% \begin{align*}
% \frac{1}{2}D_{k+1}^2 &\leq \frac{1}{2} D_k^2 - \alpha_k [f(x_{k}) + \langle \nabla f(x_k), x_{k+1} - x_k\rangle]_+ -  \frac{1}{4} \left\|x_k - x_{k+1}\right\|_{2}^2+ \alpha_k e_k +\frac{\alpha_k}{2 \eta_k}\left\|\xi_{k}\right\|_{2}^2\\
% &= \frac{1}{2} D_k^2 - (\alpha_k[f(x_{k}) + \langle \nabla f(x_k), x_{k+1} - x_k\rangle]_+ +  \frac{1}{4}\left\|x_k - x_{k+1}\right\|_{2}^2)+ \alpha_k e_k +\frac{\alpha_k}{2 \eta_k}\left\|\xi_{k}\right\|_{2}^2\\
% &\leq \frac{1}{2} D_k^2 -  (\min_y\alpha_k[f(x_{k}) + \langle \nabla f(x_k), y - x_k\rangle]_+ + \frac{1}{4} \left\|x_k -y\right\|_{2}^2)+ \alpha_k e_k +\frac{\alpha_k}{2 \eta_k}\left\|\xi_{k}\right\|_{2}^2\\
% &= \frac{1}{2} D_k^2 - (\alpha_k[f(x_{k}) - \lambda_k \| \nabla f(x_k)\|_2^2] +  \frac{\lambda_k^2}{4}  \left\| \nabla f(x_k)\right\|_{2}^2)+ \alpha_k e_k +\frac{\alpha_k}{2 \eta_k}\left\|\xi_{k}\right\|_{2}^2 \\ 
% & \hspace*{8.5cm} (\text{since } y\opt = x_k - \lambda_k \nabla f(x_k))\\
% &\leq \frac{1}{2} D_k^2 -  (\frac{1}{2}\lambda_k[f(x_{k}) - \lambda_k \| \nabla f(x_k)\|_2^2] + \frac{\lambda_k^2}{4}  \left\| \nabla f(x_k)\right\|_{2}^2)+ \alpha_k e_k +\frac{\alpha_k}{2 \eta_k}\left\|\xi_{k}\right\|_{2}^2\\
% & \hspace*{10cm} (\text{since } \lambda_k \leq 2\alpha_k)\\
% &= \frac{1}{2} D_k^2 - \frac{1}{2} \lambda_k f(x_k) + \frac{\lambda_k^2}{4} \left\|\nabla f(x_k)\right\|_{2}^2+ \alpha_k e_k +\frac{\alpha_k}{2 \eta_k}\left\|\xi_{k}\right\|_{2}^2
% \end{align*}
% We proceed by cases: if $\lambda_k = f(x_k)/ \|\nabla f(x_k)\|_{2}^2$, then $- \frac{1}{2} \lambda_k f(x_k) + \frac{\lambda_k^2}{4} \|\nabla f(x_k)\|_{2}^2 = -\frac{f(x_k)^2}{4\|\nabla f(x_k)\|_{2}^2}$. If $\lambda_k = 2\alpha_k$ (by using the fact that $2\alpha_k^2 \leq \alpha_k f(x_k) / \|\nabla f(x_k)\|_{2}^2$), then $- \frac{1}{2} \lambda_k f(x_k) + \frac{\lambda_k^2}{4} \|\nabla f(x_k)\|_{2}^2 = -\alpha_k f(x_k)/ 2$. In taking an upper bound of these two cases, we get:
% \begin{align*}
% \frac{1}{2}D_{k+1}^2 &\leq \frac{1}{2} D_k^2 - \frac{1}{2} \lambda_k f(x_k) + \frac{\lambda_k^2}{4} \left\|\nabla f(x_k)\right\|_{2}^2+ \alpha_k e_k +\frac{\alpha_k}{2 \eta_k}\left\|\xi_{k}\right\|_{2}^2\\
% &\leq  \frac{1}{2} D_k^2 - \min\left(\frac{\alpha_k f(x_k)}{2} , \frac{f(x_k)^2}{4\|\nabla f(x_k)\|_{2}^2} \right)+ \alpha_k e_k +\frac{\alpha_k}{2 \eta_k}\left\|\xi_{k}\right\|_{2}^2
% \end{align*}
% Rearranging, using Assumption \ref{assm:quad-growth}, and taking expectations on both sides, we get:
% \begin{align*}
%     \E[D_{k+1}^2] &\leq  \E[D_k^2] - \E\left[\min\left( \alpha_k f(x_k) , \frac{f(x_k)^2}{2\|\nabla f(x_k)\|_{2}^2} \right)\right]+ 2\alpha_k \E[e_k] +\frac{\alpha_k}{ \eta_k}\E[\|\xi_{k}\|_{2}^2]\\
%     &\leq  \left\{1 - \min\left(\lambda_0 \alpha_k, \frac{\lambda_1}{2} \right)  +\frac{\alpha_k \sigma^2}{m \eta_k}\right\}\E[D_k^2]
% \end{align*}
% The second inequality comes from Assumption \ref{assm:bounded-noise-dist} and the fact that $\E[e_k] \leq 0$. Now we apply the fact that $1 - t\leq e^{-t}$ to get the expression:
% \begin{align*}
%     \E[D_{k+1}^2] &\leq \left\{1 - \min\left(\lambda_0 \alpha_k, \frac{\lambda_1}{2} \right)  +\frac{\alpha_k \sigma^2}{m \eta_k}\right\}\E[D_k^2]\\
%     &\leq \exp\left\{- \min\left(\lambda_0 \alpha_k, \frac{\lambda_1}{2} \right)  +\frac{\alpha_k \sigma^2}{m \eta_k}\right\}\E[D_k^2]
% \end{align*}

% Reapplying this inequality completes the proof.



% \subsection{Proof of \Cref{prop:quad-growth-ub}}

% We have,
% \begin{align*}
%     & \E\left[(\Fbar(x;\statval) - \Fbar(x\opt;\statval))\min\left\{\stepsize,\frac{\Fbar(x;\statval) - \Fbar(x\opt,\statval)}{\ltwo{\Fbar'(x;\statval)}^2}\right\}\right] \\
%     & \geq \E\left[(\Fbar(x;\statval) - \Fbar(x\opt;\statval))\min\left\{\stepsize,\frac{\Fbar(x;\statval) - \Fbar(x\opt,\statval)}{\ltwo{\Fbar'(x;\statval)}^2}\right\}\ind{F(x;\statval) - F(x\opt;\statval) \geq c(f(x) - f(x\opt))}\right]\\
%     & \geq \E\left[(c(f(x) - f(x\opt)))\min\left\{\stepsize,\frac{c(f(x) - f(x\opt))}{\ltwo{\Fbar'(x;\statval)}^2}\right\}\ind{F(x;\statval) - F(x\opt;\statval) \geq c(f(x) - f(x\opt))}\right]
% \end{align*}
% The idea is to bound $\ltwo{\Fbar'(x;\statval)}^2$ in terms of $\ltwo{f'(x)}^2$ so as to use smoothness and get the final result. Note that, 
% \begin{align*}
%   \E[\ltwo{\Fbar'(x;\statval)}^2] &= \E[\frac{1}{m}(\ltwo{F'(x;s_i) - f'(x)) + f'(x)}^2]\\
%   & = \frac{\var(F'(x;s))}{m} + \ltwo{f'(x)}^2
% \end{align*}
% Using Markov's inequality, we have, $\P\left(\ltwo{\Fbar'(x;\statval)}^2 \leq \frac{2}{2-p} \left( \frac{\var(F'(x;s))}{m} + \ltwo{f'(x)}^2\right)\right) \geq 1 - \frac{p}{2}$. Thus,  following the calculation, we have,
% \begin{align*}
%      & \E\left[(c(f(x) - f(x\opt)))\min\left\{\stepsize,\frac{c(f(x) - f(x\opt))}{\ltwo{\Fbar'(x;\statval)}^2}\right\}\ind{F(x;\statval) - F(x\opt;\statval) \geq c(f(x) - f(x\opt))}\right] \\
%      & \geq \E\Bigg[(c(f(x) - f(x\opt)))\min\left\{\stepsize,\frac{c(f(x) - f(x\opt))}{\ltwo{\Fbar'(x;\statval)}^2}\right\}\ind{F(x;\statval) - F(x\opt;\statval) \geq c(f(x) - f(x\opt))} \\
%      &\qquad \qquad \ind{\ltwo{\Fbar'(x;\statval)}^2 \leq \frac{2}{2-p} \left( \frac{\var(F'(x;s))}{m} + \ltwo{f'(x)}^2\right)}\Bigg]\\
%      & \geq \frac{p}{2}c(f(x) - f(x\opt)) \min\left\{\alpha,\frac{c(f(x) - f(x\opt))}{\frac{2}{2-p}(\ltwo{f'(x)}^2 + \frac{\var(F'(x;s))}{m} )}\right\}\\
%      & \geq \frac{p}{2}cc_0 \min\left\{\alpha,\frac{c}{\frac{4}{2-p}(1 + \frac{\var(F'(x;s))}{m \ltwo{f'(x)}^2})L}\right\}\dist(x,\domain\opt)^2 \qquad \text{(Using L-smoothness and condition 1)}.
% \end{align*}


% \subsection{Proof of \Cref{prop:gamma-growth-lb}}
% \label{proof:prop:gamma-growth-lb}

  

% \subsection{Proof of \cref{thm:dist_opt_lam1_lb}}\label{proof:thm:dist_opt_lam1_lb}



\begin{comment}
\begin{lemma}\label{lem:risk_gamma}
Consider the problem of $(1 + \gamma)$-norm regression with loss $f_{x\opt}(x) :=\E_a[|a^T(x- x\opt)|^{1+\gamma}]$ with $a \sim\normal(0, \Gamma)$. For $\beta \in (0, 1)$ and $d-m$ large enough such that $(1 - 3e^{-\eta \beta^2 (d-m)}) > 0$, we have that:
 \[
 \mathfrak{M}(\mathcal{F},T) \geq \left((1 - 3e^{-\eta \beta^2 (d-m)}) (1 - \beta)
    \sigma\sqrt{\frac{2(d - m)}{d\pi}}\right)^{1 + \gamma}
    \]
\end{lemma}
\begin{proof}
We first lower bound the minimax risk with Bayes' risk:
\begin{align*}
    \mathfrak{M}(\mathcal{F},T) \geq \inf_{A \in \algs_T} \sup_{x\opt} \E_{a \in \R^{d}}[|a^T(x_T - x\opt)|^{1 + \gamma}] \geq \inf_{A \in \algs_T}\int \E_{a \in \R^{d}}[|a^T(x_T - x\opt)|^{1 + \gamma}] d\mu(x\opt)
\end{align*}
Some immediate facts that we know:
\begin{enumerate}
    \item For fixed $x\opt$, $f_{x\opt}(x) :=\E_a[|a^T(x- x\opt)|^{1 + \gamma}] = \E[|\normal(0, (x-x\opt)^T \Gamma (x-x\opt))|^{1 + \gamma}] \ge \E[|\normal(0, (x-x\opt)^T \Gamma (x-x\opt))|]^{1 + \gamma} = (\sqrt{\frac{2}{\pi}} \ltwo{\Gamma^{1/2}(x - x\opt)})^{1 + \gamma}$ 
    \item The posterior on $x\opt$ is $\normal(A^T(AA^T)^{-1}b,\Pi_{A^\perp} \Sigma \Pi_{A^\perp})$ where $\Pi_{A^\perp} := I - A^T(AA^T)^{-1}A$ be the projection onto $null(A)$. Which means that $x\opt - \E[x\opt |A,b]$ has $\normal(0, \Pi_{A^\perp} \Sigma \Pi_{A^\perp})$ distribution (taking expectation over $a_i$ and $A$, by tower the mean is 0).
\end{enumerate}

In particular, this means that with $Z \sim \normal(0, \Sigma)$:
\begin{align}
    \inf_{\hat x} \E_A[f_{x\opt}(\hat x)] &= \E[f_{x\opt}(\E[x\opt|A,b])] \ge \left (\sqrt{\frac{2}{\pi}}\E[\ltwo{\Gamma^{1/2}(\E[x\opt|A,b] - x\opt)}]\right)^{1 + \gamma}\\
    &= \left(\sqrt{\frac{2}{\pi}}\E_A[\ltwo{\Gamma^{1/2} \Pi_{A^\perp} Z}] \right)^{1 + \gamma}
\end{align}

Suppose that $\Gamma = \frac{1}{d} I$, then $\Pi_{A^\perp}$ is a projection onto some (uniformly) random $m$-dimensional subspace \cite{James54}. Further suppose $\Sigma = \sigma^2 I$, then we have that:

\begin{align}\label{eq:lmbda_sharp_growth_error_bound}
    \sqrt{\frac{2}{\pi}}\E_A[\ltwo{\Gamma^{1/2} \Pi_{A^\perp} Z}] &= \sigma\sqrt{\frac{2}{d\pi}}\E_A[\ltwo{\Pi_{A^\perp} N(0, I)}] \geq (1 - 3e^{-\eta \beta^2 (d-m)}) (1 - \beta)
    \sigma\sqrt{\frac{2(d - m)}{d\pi}}
\end{align}
where the $\geq$ holds by \Cref{thm:annulus} for $\beta \in (0, 1)$ when $d-m$ is sufficiently large. 
\end{proof}

\end{comment}




